Opinion Dynamics Modeling for Movie Review Transcripts Classification with Hidden Conditional Random Fields

In this paper, the main goal is to detect a movie reviewer's opinion using hidden conditional random fields. This model allows us to capture the dynamics of the reviewer's opinion in the transcripts of long unsegmented audio reviews that are analyzed by our system. High level linguistic features are computed at the level of inter-pausal segments. The features include syntactic features, a statistical word embedding model and subjectivity lexicons. The proposed system is evaluated on the ICT-MMMO corpus. We obtain a F1-score of 82\%, which is better than logistic regression and recurrent neural network approaches. We also offer a discussion that sheds some light on the capacity of our system to adapt the word embedding model learned from general written texts data to spoken movie reviews and thus model the dynamics of the opinion.

==> main <==
@article{Baccianella2010,
    title = {{SentiWordNet 3.0: An Enhanced Lexical Resource for Sentiment Analysis and Opinion Mining}},
    year = {2010},
    journal = {Proceedings of the Seventh International Conference on Language Resources and Evaluation (LREC'10)},
    author = {Baccianella, Stefano and Esuli, Andrea and Sebastiani, Fabrizio},
    number = {January},
    pages = {2200--2204},
    volume = {0},
    isbn = {2-9517408-6-7},
    doi = {citeulike-article-id:9238846}
}
@inproceedings{irsoy2014opinion,
    title = {{Opinion mining with deep recurrent neural networks}},
    year = {2014},
    booktitle = {Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
    author = {Irsoy, Ozan and Cardie, Claire},
    pages = {720--728},
    url = {http://anthology.aclweb.org/D/D14/D14-1080.pdf\nhttp://www.aclweb.org/anthology/D14-1080}
}

@article{morency2011towards,
    title = {{Towards Multimodal Sentiment Analysis: Harvesting Opinions from the Web}},
    year = {2011},
    journal = {Proceedings of the 13th International Conference on Multimodal Interfaces (ICMI-11)},
    author = {Morency, Louis-philippe and Mihalcea, Rada and Doshi, Payal},
    pages = {169--176},
    isbn = {9781450306416},
    doi = {10.1145/2070481.2070509},
    keywords = {audio-visual integration, multimodal signal processing, subjectivity and sentiment, youtube videos}
}

@article{Barras2001,
    title = {{Transcriber: Development and use of a tool for assisting speech corpora production}},
    year = {2001},
    journal = {Speech Communication},
    author = {Barras, Claude and Geoffrois, Edouard and Wu, Zhibiao and Liberman, Mark},
    number = {1-2},
    pages = {5--22},
    volume = {33},
    isbn = {3316985808},
    doi = {10.1016/S0167-6393(00)00067-4},
    issn = {01676393}
}

@inproceedings{Bousmalis2011,
    title = {{Modeling hidden dynamics of multimodal cues for spontaneous agreement and disagreement recognition}},
    year = {2011},
    booktitle = {2011 IEEE International Conference on Automatic Face and Gesture Recognition and Workshops, FG 2011},
    author = {Bousmalis, Konstantinos and Morency, Louis-Philippe and Pantic, Maja},
    pages = {746--752},
    isbn = {9781424491407},
    doi = {10.1109/FG.2011.5771341}
}

@inproceedings{Campione2002,
    title = {{A large-scale multilingual study of pause duration}},
    year = {2002},
    booktitle = {Speech Prosody 2002. Proceedings of the1st International Conference on Speech Prosody},
    author = {Campione, Estelle and V{\'{e}}ronis, Jean},
    pages = {199--202},
    url = {http://www.isca-speech.org/archive/sp2002/sp02_199.html},
    doi = {10.1.1.12.561}
}


@article{Schuller2009,
    title = {{"The Godfather" vs. "Chaos": Comparing linguistic analysis based on on-line knowledge sources and bags-of-N-grams for movie review valence estimation}},
    year = {2009},
    journal = {Proceedings of the International Conference on Document Analysis and Recognition, ICDAR},
    author = {Schuller, Bjorn and Schenk, Joachim and Rigoll, Gerhard and Knaup, Tobias},
    pages = {858--862},
    isbn = {9780769537252},
    doi = {10.1109/ICDAR.2009.194},
    issn = {15205363}
}

@misc{Chollet2015,
    title = {{Keras}},
    year = {2015},
    author = {Chollet, Francois},
    url = {https://github.com/fchollet/keras}
}


@article{Hochreiter1997,
    title = {{LONG SHORT-TERM MEMORY}},
    year = {1997},
    journal = {Neural Computation},
    author = {Hochreiter, Sepp and Urgen Schmidhuber, J},
    number = {8},
    pages = {1735--1780},
    volume = {9},
    url = {http://www7.informatik.tu-muenchen.de/~hochreit%5Cnhttp://www.idsia.ch/~juergen},
    isbn = {08997667 (ISSN)},
    doi = {10.1162/neco.1997.9.8.1735},
    issn = {0899-7667},
    pmid = {9377276},
    arxivId = {1206.2944}
}

@article{Kingma2014,
    title = {{Adam: A Method for Stochastic Optimization}},
    year = {2014},
    journal = {International Conference on Learning Representations},
    author = {Kingma, Diederik and Ba, Jimmy},
    pages = {1--13},
    url = {http://arxiv.org/abs/1412.6980},
    isbn = {9781450300728},
    doi = {http://doi.acm.org.ezproxy.lib.ucf.edu/10.1145/1830483.1830503},
    issn = {09252312},
    arxivId = {1412.6980}
}

@inproceedings{Bousmalis2011,
    title = {{Modeling hidden dynamics of multimodal cues for spontaneous agreement and disagreement recognition}},
    year = {2011},
    booktitle = {2011 IEEE International Conference on Automatic Face and Gesture Recognition and Workshops, FG 2011},
    author = {Bousmalis, Konstantinos and Morency, Louis-Philippe and Pantic, Maja},
    pages = {746--752},
    isbn = {9781424491407},
    doi = {10.1109/FG.2011.5771341}
}

@misc{Piglet,
    title = {{Spell Checker}},
    author = {McCallum, Jonas},
    url = {https://github.com/phatpiglet/autocorrect}
}

@inproceedings{Kennedy2006,
    title = {{Sentiment classification of movie reviews using contextual valence shifters}},
    year = {2006},
    booktitle = {Computational Intelligence},
    author = {Kennedy, Alistair and Inkpen, Diana},
    number = {2},
    pages = {110--125},
    volume = {22},
    isbn = {1467-8640},
    doi = {10.1111/j.1467-8640.2006.00277.x},
    issn = {08247935},
    keywords = {Evaluation, Machine learning, Semantic orientation, Sentiment classification, Valence shifters}
}

@article{Mikolov2013,
    title = {{Efficient Estimation of Word Representations in Vector Space}},
    year = {2013},
    journal = {Proceedings of the International Conference on Learning Representations (ICLR 2013)},
    author = {Mikolov, Tomas and Corrado, Greg and Chen, Kai and Dean, Jeffrey},
    pages = {1--12},
    url = {http://arxiv.org/pdf/1301.3781v3.pdf},
    isbn = {1532-4435},
    doi = {10.1162/153244303322533223},
    issn = {15324435},
    pmid = {18244602},
    arxivId = {arXiv:1301.3781v3}
}


@article{Mikolov2013b,
    title = {{Linguistic regularities in continuous space word representations}},
    year = {2013},
    journal = {Proceedings of NAACL-HLT},
    author = {Mikolov, Tomas and Yih, Wen-tau and Zweig, Geoffrey},
    number = {June},
    pages = {746--751},
    url = {http://scholar.google.com/scholar?hl=en&btnG=Search&q=intitle:Linguistic+Regularities+in+Continuous+Space+Word+Representations#0%5Cnhttps://www.aclweb.org/anthology/N/N13/N13-1090.pdf},
    isbn = {9781937284473},
    pmid = {1938007}
}

@inproceedings{Mikolov2013a,
    title = {{Distributed Representations of Words and Phrases and their Compositionality}},
    year = {2013},
    booktitle = {Proc. NIPS},
    author = {Mikolov, Tomas and Sutskever, I. and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
    pages = {1--9},
    isbn = {2150-8097},
    doi = {10.1162/jmlr.2003.3.4-5.951},
    issn = {10495258},
    pmid = {903},
    arxivId = {1310.4546}
}


@misc{Morency2007,
    title = {{Hidden-state Conditional Random Field (HCRF) Library}},
    year = {2007},
    author = {Morency, Louis-Philippe},
    url = {http://sourceforge.net/projects/hcrf/}
}

@article{Pedregosa2012,
    title = {{Scikit-learn: Machine Learning in Python}},
    year = {2012},
    journal = {Journal of Machine Learning Research},
    author = {Pedregosa, Fabian and Varoquaux, Gaël and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and Vanderplas, Jake and Passos, Alexandre and Cournapeau, David and Brucher, Matthieu and Perrot, Matthieu and Duchesnay, Édouard},
    pages = {2825--2830},
    volume = {12},
    url = {http://dl.acm.org/citation.cfm?id=2078195%5Cnhttp://arxiv.org/abs/1201.0490},
    isbn = {1532-4435},
    doi = {10.1007/s13398-014-0173-7.2},
    issn = {15324435},
    pmid = {1000044560},
    arxivId = {1201.0490}
}


@article{Perez-Rosas2013,
    title = {{Utterance-Level Multimodal Sentiment Analysis}},
    year = {2013},
    journal = {Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
    author = {Perez-Rosas, Veronica and Mihalcea, Rada and Morency, Louis-Philippe},
    pages = {973--982},
    url = {http://www.aclweb.org/anthology/P13-1096},
    isbn = {9781937284503}
}


@inproceedings{Poria2015a,
    title = {{Deep Convolutional Neural Network Textual Features and Multiple Kernel Learning for Utterance-level Multimodal Sentiment Analysis}},
    year = {2015},
    booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing},
    author = {Poria, Soujanya and Cambria, Erik and Gelbukh, Alexander},
    pages = {2539–2544},
    url = {http://aclweb.org/anthology/D15-1303},
    isbn = {9781941643327}
}


@article{Poria2016,
    title = {{Fusing audio, visual and textual clues for sentiment analysis from multimodal content}},
    year = {2016},
    journal = {Neurocomputing},
    author = {Poria, Soujanya and Cambria, Erik and Howard, Newton and Huang, Guang Bin and Hussain, Amir},
    pages = {50--59},
    volume = {174},
    publisher = {Elsevier},
    url = {http://dx.doi.org/10.1016/j.neucom.2015.01.095},
    isbn = {0925-2312},
    doi = {10.1016/j.neucom.2015.01.095},
    issn = {18728286},
    keywords = {Big social data analysis, Multimodal fusion, Multimodal sentiment analysis, Opinion mining, Sentic computing}
}



@article{Quattoni2007,
    title = {{Hidden conditional random fields.}},
    year = {2007},
    journal = {IEEE transactions on pattern analysis and machine intelligence},
    author = {Quattoni, Ariadna and Wang, Sybor and Morency, Louis-Philippe and Collins, Michael and Darrell, Trevor},
    number = {10},
    pages = {1848--1853},
    volume = {29},
    isbn = {0162-8828},
    doi = {10.1109/TPAMI.2007.1124},
    issn = {0162-8828},
    pmid = {17699927}
}

@article{Schuster2016,
    title = {{Enhanced English Universal Dependencies: An Improved Representation for Natural Language Understanding Tasks}},
    year = {2016},
    journal = {Proceedings of the Tenth International Conference on Language Resources and Evaluation (LREC 2016)},
    author = {Schuster, Sebastian and Manning, Christopher D.},
    pages = {2371--2378},
    url = {http://nlp.stanford.edu/~sebschu/pubs/schuster-manning-lrec2016.pdf},
    keywords = {semantic representation, treebank conversion, universal dependencies}
}


@article{Socher2013,
    title = {{Recursive deep models for semantic compositionality over a sentiment treebank}},
    year = {2013},
    journal = {EMNLP-2013: Conference on Empirical Methods in Natural Language Processing},
    author = {Socher, Richard and Perelygin, Alex and Wu, Jy},
    pages = {1631--1642},
    url = {http://nlp.stanford.edu/~socherr/EMNLP2013_RNTN.pdf%5Cnhttp://www.aclweb.org/anthology/D13-1170%5Cnhttp://aclweb.org/supplementals/D/D13/D13-1170.Attachment.pdf%5Cnhttp://oldsite.aclweb.org/anthology-new/D/D13/D13-1170.pdf},
    isbn = {9781937284978},
    doi = {10.1371/journal.pone.0073791},
    issn = {1932-6203},
    pmid = {24086296},
    arxivId = {1512.03385}
}

@article{Taboada2011,
    title = {{Lexicon-Based Methods for Sentiment Analysis}},
    year = {2011},
    journal = {Computational Linguistics},
    author = {Taboada, Maite and Brooke, Julian and Tofiloski, Milan and Voll, Kimberly and Stede, Manfred},
    number = {2},
    pages = {267--307},
    volume = {37},
    isbn = {0891-2017},
    doi = {10.1162/COLI{\_}a{\_}00049},
    issn = {0891-2017}
}


@article{Wagner2014,
    title = {{DCU: Aspect-based Polarity Classification for SemEval Task 4}},
    year = {2014},
    journal = {Proceedings of the 8th International Workshop on Semantic Evaluation (SemEval 2014)},
    author = {Wagner, Joachim and Arora, Piyush and Cortes, Santiago and Barman, Utsab and Bogdanova, Dasha and Foster, Jennifer and Tounsi, Lamia},
    number = {SemEval},
    pages = {223--229},
    url = {http://www.aclweb.org/anthology/S14-2036}
}

@article{Warriner2013,
    title = {{Norms of valence, arousal, and dominance for 13,915 English lemmas}},
    year = {2013},
    journal = {Behavior Research Methods},
    author = {Warriner, Amy Beth and Kuperman, Victor and Brysbaert, Marc},
    number = {4},
    pages = {1191--1207},
    volume = {45 VN - r},
    url = {http://www.ncbi.nlm.nih.gov/pubmed/23404613%5Cnhttp://dx.doi.org/10.3758/s13428-012-0314-x},
    isbn = {1554-351X},
    doi = {10.3758/s13428-012-0314-x},
    issn = {1554-3528},
    pmid = {23404613},
    keywords = {80 and over, Adolescent, Adult, Affect, Aged, Arousal, Arousal: physiology, Crowdsourcing, Crowdsourcing: methods, Databases, Educational Status, Emotions, Emotions: physiology, European Continental Ancestry Group, Factual, Female, Humans, Male, Middle Aged, Reading, Reference Values, Semantics, Sesquiterpenes, Sex Characteristics, Social Dominance, Socioeconomic Factors, Vocabulary, Word Association Tests, Word Association Tests: standards, Young Adult}
}

@article{wollmer2013youtube,
    title = {{YouTube Movie Reviews: Sentiment Analysis in an Audio-Visual Context}},
    year = {2013},
    journal = {IEEE Intelligent Systems},
    author = {W{\"{o}}llmer, Martin and Weninger, Felix and Knaup, Tobias and Schuller, Bjorn and Sun, Congkai and Sagae, Kenji and Morency, Louis-Philippe},
    number = {3},
    pages = {46--53},
    volume = {28},
    url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=6487473},
    isbn = {1541-1672 VO - 28},
    doi = {10.1109/MIS.2013.34},
    issn = {1541-1672},
    keywords = {Context awareness, Feature extraction, Motion pictures, Pragmatics, Videos, Visualization, YouTube, YouTube movie reviews, affective computing, audio-visual context, audio-visual pattern recognition, audio-visual systems, emotion recognition, entertainment, intelligent systems, linguistic analysis, linguistics, online videos, reviews, sentiment analysis, social networking (online), speech processing, speech-based emotion recognition, textual information, video signal processing}
}

@article{yang2013joint,
    title = {{Joint Inference for Fine-grained Opinion Extraction}},
    year = {2013},
    journal = {Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics,},
    author = {Yang, Bishan and Cardie, Claire},
    pages = {1640--1649},
    isbn = {9781937284503}
}





